Piecewise Linear Equivariant Maps for Compact Groups

Motivated by equivariant neural networks, we study piecewise linear equivariant maps between finite-dimensional real representations of compact groups. We show that all genuinely non-linear piecewise linear behaviour is confined to the subspaces on which the identity component of the group acts trivially, while equivariance forces linearity on the corresponding orthogonal complements. As a consequence, we obtain a compact-group analogue of the finite-group existence criterion of Gibson--Tubbenhauer--Williamson for non-zero equivariant piecewise linear maps between irreducible representations, with the identity component giving rise to a rigidity phenomenon absent from the finite-group case.

==> bib.tex <==

%\begin{bibdiv}
\begin{biblist}

%\bib{ABLS}{article}{
%author={Afsar, Zahra},
%author={Brownlowe, Nathan},
%author={Larsen, Nadia S.},
%author={Stammeier, Nicolai},
%title={Equilibrium states on right LCM semigroup $C^*$-algebras},
%journal={Int. Math. Res. Not.},
%year={2017 (advance article)},
%doi={\href{https://doi.org/10.1093/imrn/rnx162}{10.1093/imrn/rnx162}},
%%note={preprint, \href{https://arxiv.org/abs/1611.01052}{arxiv:1611.01052}},
%}

\bib{ALV}{article}{
  title={Interacting Fock spaces and Hilbert module extensions of the Heisenberg commutation relations},
  author={Accardi, Luigi},
  author={Lu, Yun-Gang},
  author={Volovich, Igor},
  journal={Publications of IIAS, Kyoto},
  year={1997}
}


\bib{A}{article}{
AUTHOR = {Aiello, Valeriano},
TITLE = {On the {A}lexander theorem for the oriented Thompson group
  {$\vec{F}$}},
JOURNAL = {Algebr. Geom. Topol.},
FJOURNAL = {Algebraic \& Geometric Topology},
VOLUME = {20},
YEAR = {2020},
NUMBER = {1},
PAGES = {429--438},
ISSN = {1472-2747},
MRCLASS = {57K10},
MRNUMBER = {4071378},
MRREVIEWER = {Masakazu Teragaito},
DOI = {10.2140/agt.2020.20.429},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.2140/agt.2020.20.429},
}

\bib{A2}{article}{ 
title={An introduction to Thompson knot theory and to Jones subgroups},
author={Aiello, Valeriano},
journal={J. Knot Theory Ramifications, preprint arXiv:2211.15461},
year={2022}
}



\bib{AB1}{article}{
author={Aiello, Valeriano},
author={Baader, Sebastian},
title={Positive oriented Thompson links},
note={accepted for publication in Communications in Analysis and Geometry, preprint \href{http://arxiv.org/abs/2101.04534}{arXiv:2101.04534}},
year={2021},
}


\bib{AB2}{article}{
title={Arborescence of positive Thompson links},
author={Aiello, Valeriano},
author={Baader, Sebastian}, 
note={preprint \href{http://arxiv.org/abs/2106.13648}{arXiv:2106.13648}},
journal={Pacific Journal of Mathematics},
volume={316} 
issue={2}, 
pages={237-248}, 
year={2022}
}



\bib{ABC}{article}{
author={Aiello, Valeriano},
author={Brothier, Arnaud},
author={Conti, Roberto},
title={Jones representations of Thompson's group $F$ arising from Temperley-Lieb-Jones algebras},
journal={Int. Math. Res. Not.},
VOLUME = {15},
PAGES = {11209-11245},
year={2021},
doi={https://doi.org/10.1093/imrn/rnz240},
note={preprint \href{http://arxiv.org/abs/1901.10597}{arXiv:1901.10597}},
%year={2016},
}
%Int. Math. Res. Not. 15 (2021), 11209–11245, doi: 10.1093/imrn/rnz240 
		

\bib{AiCo1}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
TITLE = {Graph polynomials and link invariants as positive type
  functions on {T}hompson's group {$F$}},
JOURNAL = {J. Knot Theory Ramifications},
FJOURNAL = {Journal of Knot Theory and its Ramifications},
VOLUME = {28},
YEAR = {2019},
NUMBER = {2},
PAGES = {1950006, 17},
ISSN = {0218-2165},
MRCLASS = {43A35 (05C31 57M27)},
MRNUMBER = {3924840},
MRREVIEWER = {Markus Neuhauser},
DOI = {10.1142/S0218216519500068},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1142/S0218216519500068},
}


\bib{AiCo2}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
TITLE = {The Jones polynomial and functions of positive type on the
  oriented Jones-Thompson groups {$\vec {F}$} and {$\vec
  {T}$}},
JOURNAL = {Complex Anal. Oper. Theory},
FJOURNAL = {Complex Analysis and Operator Theory},
VOLUME = {13},
YEAR = {2019},
NUMBER = {7},
PAGES = {3127--3149},
ISSN = {1661-8254},
MRCLASS = {57M27 (05C31 43A35)},
MRNUMBER = {4020028},
DOI = {10.1007/s11785-018-0866-6},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s11785-018-0866-6},
}		


\bib{ACR1}{article}{
  title={A look at the inner structure of the 2-adic ring C$^*$-algebra and its automorphism groups},
  author={Aiello, Valeriano},
  author={Conti, Roberto},
  author={Rossi, Stefano},
  journal={Publications of the Research Institute for Mathematical Sciences},
  volume={54},
  number={1},
  pages={45--87},
  year={2018},
  publisher={European Mathematical Society Publishing House}
}

\bib{ACR4}{article}{
  title={Normalizers and permutative endomorphisms of the 2-adic ring C$^*$-algebra},
author={Aiello, Valeriano},
  author={Conti, Roberto},
  author={Rossi, Stefano}, 
   journal={Journal of Mathematical Analysis and Applications},
  volume={481},
  number={1},
  pages={123395},
  year={2020},
  publisher={Elsevier}
}


\bib{ACRsurvey}{article}{
  title={A hitchhiker’s guide to endomorphisms and automorphisms of Cuntz algebras},
author={Aiello, Valeriano},
  author={Conti, Roberto},
  author={Rossi, Stefano},
    journal={Rend. Mat. Appl},
  volume={42},
  pages={61--162},
  year={2021}
}



\bib{ACJ}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {The Homflypt polynomial and the oriented Thompson group},
JOURNAL = {Quantum Topol.},
FJOURNAL = {Quantum Topology},
VOLUME = {9},
YEAR = {2018},
NUMBER = {3},
PAGES = {461--472},
ISSN = {1663-487X},
MRCLASS = {57M27 (20F65)},
MRNUMBER = {3827807},
MRREVIEWER = {Bruno P. Zimmermann},
DOI = {10.4171/QT/112},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/QT/112},
}
		






\bib{AJ}{article}{
AUTHOR = {Aiello, Valeriano}, % and Jones, Vaughan F. R.},
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {On spectral measures for certain unitary representations of
  {R}. {T}hompson's group {F}},
JOURNAL = {J. Funct. Anal.},
FJOURNAL = {Journal of Functional Analysis},
VOLUME = {280},
YEAR = {2021},
NUMBER = {1},
PAGES = {108777, 27},
ISSN = {0022-1236},
MRCLASS = {22D10 (18M30 20F65 46L37)},
MRNUMBER = {4156130},
DOI = {10.1016/j.jfa.2020.108777},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jfa.2020.108777},
}

\bib{TV}{article}{
author={Aiello, Valeriano},
author={Nagnibeda, Tatiana},
title={On the oriented Thompson subgroup $\vec{F}_3$ and its relatives in higher Brown-Thompson groups},
journal={Journal of Algebra and its Applications},
volume={21}, 
number={07}, 
note={2250139, preprint \href{http://arxiv.org/abs/1912.04730}{arXiv:1912.04730}},
year={2022},
}


\bib{TV2}{article}{
author={Aiello, Valeriano},
author={Nagnibeda, Tatiana},
title={On the 3-colorable subgroup $\mathcal{F}$ and maximal subgroups of Thompson’s group $F$},
journal={Annales l'Institut Fourier},
volume={73},
number={2},
pages={783--828},
year={2023},
note={preprint \href{http://arxiv.org/abs/2103.07885}{arXiv:2103.07885}},
} 


\bib{TV3}{article}{
title={The planar $3$-colorable subgroup $\mathcal E$  of Thompson's group $F$ and its even part},
author={Aiello, Valeriano},
author={Nagnibeda, Tatiana},
journal={Proceedings of the Edinburgh Mathematical Society, preprint arXiv:2212.12269},
year={2022}
}



\bib{AP}{article}{ 
title={Representations of Higman-Thompson groups from Cuntz algebras},
author={Ara{\'u}jo, Francisco},
author={Pinto, Paulo R.},
title={Representations of Higman-Thompson groups from Cuntz algebras},
journal={Journal of Mathematical Analysis and Applications},
volume = {509},
number = {2},
pages = {125970},
year = {2022},
publisher={Elsevier}
%  note={preprint \href{http://arxiv.org/abs/2011.13679}{arXiv:2011.13679}},
%  journal={preprint arXiv:2011.13679},
%year={2020}
}


\bib{AK}{article}{
  title={Gysin sequences and $SU(2)$-symmetries of C$^*$-algebras},
  author={Arici, Francesca},
  author={Kaad, Jens},
  journal={Transactions of the London Mathematical Society},
  volume={8},
  number={1},
  pages={440--492},
  year={2021},
  publisher={Wiley Online Library}
}

\bib{Nesh3}{article}{
  title={KK-duality for the Cuntz-Pimsner algebras of Temperley-Lieb subproduct systems},
  author={Arici, Francesca},
  author={Gerontogiannis, Dimitris},
  author={Neshveyev, Sergey},
  journal={preprint arXiv:2401.01725},
  year={2024}
}



\bib{Arveson98}{article}{
 Author = {Arveson, William},
 Title = {Subalgebras of C$^*$-algebras. III: Multivariable operator theory},
 %FJournal = {Acta Mathematica},
 Journal = {Acta Math.},
 %ISSN = {0001-5962},
 Volume = {181},
 Number = {2},
 Pages = {159--228},
 Year = {1998},
 %Language = {English},
 DOI = {10.1007/BF02392585},
 %Keywords = {46L05,47L80},
% zbMATH = {1269879},
% Zbl = {0952.46035}
}


\bib{BadNip}{book}{%baader1998term,
title={Term rewriting and all that},
author={Baader, Franz},
author={Nipkow, Tobias},
year={1998},
publisher={Cambridge university press}
}


\bib{SavBak}{article}{
title={Explicit Generators for the Stabilizers of Rational Points in Thompson's Group $ F$},
author={Baker, Krystofer},
author={Savchuk, Dmytro},
journal={preprint arXiv:2401.00404},
year={2023}
}

\bib{BP}{article}{ 
title={Representations of Thompson groups from Cuntz algebras},
author={Barata, Miguel},
author={Pinto, Paulo R.},
journal={Journal of Mathematical Analysis and Applications},
volume = {478},
number = {1},
pages = {212-228},
year = {2019},%doi = {https://doi.org/10.1016/j.jmaa.2021.125970},
publisher={Elsevier}
}


\bib{BOS18}{article}{ 
  title={On the K-theory of C$^*$-algebras arising from integral dynamical systems},
  author={Barlak, Sel\c{c}uk },
  author={Omland, Tron},
  author={Stammeier, Nicolai},
  journal={Ergod. Thy. \& Dynam. Sys},
  volume={38},
  pages={832--862},
  year={2018}
}



\bib{BDVRV}{article}{
  title={Neural reproducing kernel Banach spaces and representer theorems for deep networks},
  author={Bartolucci, Francesca},
  author={De Vito, Ernesto},
  author={Rosasco, Lorenzo},
  author={Vigogna, Stefano},
  journal={preprint arXiv:2403.08750},
  year={2024}
}



\bib{BPRS}{article}{ 
title = {The C$^*$-algebras of row-finite graphs},
author= {Bates, Teresa},
 author = {Pask, David},
 author = {Raeburn, Iain},
 author = {Szyma{\'n}ski, Wojciech},
 journal = {New York J. Math.},
 ISSN = {1076-9803},
 Volume = {6},
 Pages = {307--324},
 Year = {2000},
% Language = {English},
% Keywords = {46L05,05C20},
% zbMATH = {1531353},
% Zbl = {0976.46041}
}

\bib{Bhat}{article}{ 
  title={Inclusion systems and amalgamated products of product systems},
  author={Bhat, BV Rajarama},
  author={Mukherjee, Mithun},
  journal={Infinite Dimensional Analysis, Quantum Probability and Related Topics},
  volume={13},
  number={01},
  pages={1--26},
  year={2010},
  publisher={World Scientific}
}


\bib{B}{article}{
title={Thompson's group F},
author={Belk, James},
note={preprint \href{http://arxiv.org/abs/0708.3609}{arXiv:0708.3609}},
%  journal={preprint arXiv:0708.3609},
year={2007}
}

\bib{BBQS}{article}{
title={Type systems and maximal subgroups of Thompson's group $ V$},
author={Belk, James},
author={Bleak, Collin},
author={Quick, Martyn},
author={Skipper, Rachel},
journal={preprint arXiv:2206.12631},
year={2022}
}


\bib{BM}{article}{
AUTHOR = {Belk, James},
AUTHOR = {Matucci, Francesco},
TITLE = {Conjugacy and dynamics in Thompson's groups},
JOURNAL = {Geom. Dedicata},
FJOURNAL = {Geometriae Dedicata},
VOLUME = {169},
YEAR = {2014},
PAGES = {239--261},
ISSN = {0046-5755},
MRCLASS = {20F65},
MRNUMBER = {3175247},
MRREVIEWER = {Dmytro M. Savchuk},
DOI = {10.1007/s10711-013-9853-2},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s10711-013-9853-2},
}

\bib{Halverson}{article}{
  title={Motzkin algebras},
  author={Benkart, Georgia},
  author={Halverson, Tom},
  journal={European Journal of Combinatorics},
  volume={36},
  pages={473--502},
  year={2014},
  publisher={Elsevier}
}



\bib{Bil}{book}{%billingsley2017probability,
title={Probability and measure},
author={Billingsley, Patrick},
year={2017},
publisher={John Wiley \& Sons}
}


\bib{BW}{article}{
author={Bleak, Collin},
author={Wassink, Bronlyn},
title={Finite index subgroups of R. Thompson's group F},
note={preprint \href{http://arxiv.org/abs/0711.1014}{arXiv:0711.1014}},
year={2007},
}

\bib{Bro0}{article}{
title={On Jones' connections between subfactors, conformal field theory, Thompson's groups and knots},
author={Brothier, Arnaud},
journal={preprint arXiv:1912.07140},
year={2019}
}


\bib{Bro1}{article}{
title={Forest-skein groups I: between Vaughan Jones' subfactors and Richard Thompson's groups},
author={Brothier, Arnaud},
journal={preprint arXiv:2207.03100},
year={2022}
}


\bib{Bro2}{article}{
title={Forest-skein groups II: Construction from homogeneously presented monoids},
author={Brothier, Arnaud},
journal={International Journal of Mathematics},
volume={34},
number={08},
pages={2350042},
year={2023},
publisher={World Scientific}
}


\bib{BJ}{article}{
AUTHOR = {Brothier, Arnaud},
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {Pythagorean representations of Thompson's groups},
JOURNAL = {J. Funct. Anal.},
FJOURNAL = {Journal of Functional Analysis},
VOLUME = {277},
YEAR = {2019},
NUMBER = {7},
PAGES = {2442--2469},
ISSN = {0022-1236},
MRCLASS = {22D25 (20F65 46L05)},
MRNUMBER = {3989149},
MRREVIEWER = {Bachir Bekka},
DOI = {10.1016/j.jfa.2019.02.009},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jfa.2019.02.009},
}
		

\bib{BJ2}{article}{
AUTHOR = {Brothier, Arnaud},
AUTHOR = {Jones, Vaughan F. R.},
title={On the Haagerup and Kazhdan properties of R. Thompson’s groups},
journal={Journal of Group Theory},
volume={22},
number={5},
pages={795--807},
year={2019}
}


\bib{BrWi}{article}{
title={Jones' representations of R. Thompson's groups not induced by finite-dimensional ones},
author={Brothier, Arnaud},
author={Wijesena, Dilshan},
journal={preprint arXiv:2211.08555},
year={2022}
}


\bib{Brown}{article}{
AUTHOR = {Brown, Kenneth S.},
TITLE = {Finiteness properties of groups},
BOOKTITLE = {Proceedings of the {N}orthwestern conference on cohomology of
  groups ({E}vanston, {I}ll., 1985)},
JOURNAL = {J. Pure Appl. Algebra},
FJOURNAL = {Journal of Pure and Applied Algebra},
VOLUME = {44},
YEAR = {1987},
NUMBER = {1-3},
PAGES = {45--75},
ISSN = {0022-4049},
MRCLASS = {20J05 (11F75 20F05 22E40)},
MRNUMBER = {885095},
MRREVIEWER = {Ralph Strebel},
DOI = {10.1016/0022-4049(87)90015-6},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/0022-4049(87)90015-6},
}

\bib{BCS}{article}{
title={Metrics and embeddings of generalizations of Thompson’s group F},
author={Burillo, Jos{\'e}},
author={Cleary, Sean},
author={Stein, Melanie},
journal={Transactions of the American Mathematical Society},
volume={353},
number={4},
pages={1677--1689},
year={2001}
}

\bib{CFP}{article}{
author={Cannon, James W.},
author={Floyd, William J.},  
author={Parry, Walter R.},
TITLE = {Introductory notes on Richard Thompson's groups},
JOURNAL = {Enseign. Math. (2)},
FJOURNAL = {L'Enseignement Math\'{e}matique. Revue Internationale. 2e S\'{e}rie},
VOLUME = {42},
YEAR = {1996},
NUMBER = {3-4},
PAGES = {215--256},
ISSN = {0013-8584},
MRCLASS = {20F32 (57M07)},
MRNUMBER = {1426438},
MRREVIEWER = {Michael L. Mihalik},
}

\bib{Cohen18}{article}{ 
  title={Spherical CNNs},
  author={Cohen, Taco S },
  author={Geiger, Mario},
  author={K{\"o}hler, Jonas},
  author={Welling, Max},
  journal={preprint arXiv:1801.10130},
  year={2018}
}



\bib{CR}{article}{
  title={Failure of the Ryll-Nardzewski theorem on the CAR algebra},
  author={Crismale, Vitonofrio},
  author={Rossi, Stefano},
  journal={Journal of Functional Analysis},
  volume={283},
  number={12},
  pages={109710},
  year={2022},
  publisher={Elsevier}
}

\bib{CDR}{article}{,
  title={On distributional symmetries on the CAR algebra},
  author={Crismale, Vitonofrio},
  author={Del Vecchio, Simone},
  author={Rossi, Stefano},
    journal={preprint arXiv:2209.05431},
  year={2022}
}


\bib{Cuntz}{article}{ 
title={Simple C$^*$-algebra generated by isometries},
author={Cuntz, Joachim},
journal={Communications in mathematical physics},
volume={57},
number={2},
pages={173--185},
year={1977},
publisher={Springer}
}


\bib{Cybenko89}{article}{
  title={Approximation by superpositions of a sigmoidal function},
  author={Cybenko, George},
  journal={Mathematics of control, signals and systems},
  volume={2},
  number={4},
  pages={303--314},
  year={1989},
  publisher={Springer}
}


\bib{Cybenko89err}{article}{
  title={Correction Approximation by Superpositions of a Sigmoidal Function},
  author={Cybenko, George},
  journal={Mathematics of control, signals and systems},
  volume={5},
   pages={455},
  year={1992},
  publisher={Springer}
} 


\bib{DM}{article}{
AUTHOR = {Dudko, Artem},
AUTHOR = {Medynets, Konstantin},
TITLE = {Finite factor representations of Higman-Thompson groups},
JOURNAL = {Groups Geom. Dyn.},
FJOURNAL = {Groups, Geometry, and Dynamics},
VOLUME = {8},
YEAR = {2014},
NUMBER = {2},
PAGES = {375--389},
ISSN = {1661-7207},
MRCLASS = {20C15 (22F10 37A05)},
MRNUMBER = {3231220},
MRREVIEWER = {Nhan-Phu Chung},
DOI = {10.4171/GGD/230},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/GGD/230},
}
	
	
	
\bib{DF}{article}{
title={On the stabilisers of points in groups with micro-supported actions},
author={Francoeur, Dominik},
journal = {Journal of Group Theory},
number = {3},
volume = {24},
year = {2021},
pages = {533--547}
publisher={De Gruyter}
}

\bib{HofmannMorris}{book}{ 
  title={The structure of compact groups: a primer for the student, a handbook for the expert},
  author={Hofmann, Karl Heinrich},
  author={Morris, Sidney A.},
  volume={13},
  year={2006},
  publisher={Walter de Gruyter Berlin}
}



\bib{GerholdSkeide}{article}{
  title={Interacting Fock spaces and subproduct systems},
  author={Gerhold, Malte},
  author={Skeide, Michael},
  journal={Infinite Dimensional Analysis, Quantum Probability and Related Topics},
  volume={23},
  number={03},
  pages={2050017},
  year={2020},
  publisher={World Scientific}
}	
	
	
	
\bib{Gibson24}{article}{ 
  title={Equivariant neural networks and piecewise linear representation theory},
  author={Gibson, Joe},
  author={ Tubbenhauer, Daniel},
    author={Williamson, Geordie},
  journal={Contemp. Math.}, % preprint arXiv:2408.00949},
    volume={829},
  pages={157-192},
  year={2025}
}
	
	
\bib{G}{article}{
title={The generation problem in Thompson group $ F$},
author={Golan, Gili},
preprint={arXiv:1608.02572},
year={2016}
}



\bib{G2}{article}{
title={On Maximal Subgroups of Thompson's Group $F$},
author={Golan, Gili},
journal={preprint arXiv:2209.03244},
year={2022}
}



\bib{GS}{article}{
AUTHOR = {Golan, Gili}, 
AUTHOR = {Sapir, Mark},    
TITLE = {On {J}ones' subgroup of {R}. {T}hompson group {$F$}},
JOURNAL = {J. Algebra},
FJOURNAL = {Journal of Algebra},
VOLUME = {470},
YEAR = {2017},
PAGES = {122--159},
ISSN = {0021-8693},
MRCLASS = {20F65 (20F05 57M25)},
MRNUMBER = {3565428},
MRREVIEWER = {J. S. Birman},
DOI = {10.1016/j.jalgebra.2016.09.001},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jalgebra.2016.09.001},
}
	
\bib{GS2}{article}{
AUTHOR = {Golan, Gili}, 
AUTHOR = {Sapir, Mark},
TITLE = {On subgroups of {R}. {T}hompson's group {$F$}},
JOURNAL = {Trans. Amer. Math. Soc.},
FJOURNAL = {Transactions of the American Mathematical Society},
VOLUME = {369},
YEAR = {2017},
NUMBER = {12},
PAGES = {8857--8878},
ISSN = {0002-9947},
MRCLASS = {20F65 (20G07)},
MRNUMBER = {3710646},
MRREVIEWER = {J. S. Birman},
DOI = {10.1090/tran/6982},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1090/tran/6982},
}

\bib{GS3}{article}{
AUTHOR = {Golan, Gili}, 
AUTHOR = {Sapir, Mark},
TITLE = {On the stabilizers of finite sets of numbers in the {R}.
  {T}hompson group {$F$}},
JOURNAL = {Algebra i Analiz},
FJOURNAL = {Rossi\u{\i}skaya Akademiya Nauk. Algebra i Analiz},
VOLUME = {29},
YEAR = {2017},
NUMBER = {1},
PAGES = {70--110},
ISSN = {0234-0852},
MRCLASS = {20F38 (20F05)},
MRNUMBER = {3660685},
DOI = {10.1090/spmj/1482},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1090/spmj/1482},
}
		
		
\bib{GS4}{article}{
title={On closed subgroups of the R. Thompson group $F$},
AUTHOR = {Golan, Gili}, 
AUTHOR = {Sapir, Mark},  
note={preprint \href{http://arxiv.org/abs/2105.00531}{arXiv:2105.00531}},    
%   journal={preprint arXiv:2105.00531},
year={2021}
}

\bib{Gri}{article}{
  title={On maximal subgroups of ample groups},
  author={Grigorchuk, Rostislav},
  author={Vorobets, Yaroslav},
  journal={preprint arXiv:2403.16364},
  year={2024}
}


\bib{Grigsby25}{article}{ 
  title={Functional dimension of feedforward ReLU neural networks},
  author={Grigsby, Julia Elisenda},
  author={Lindsey, Kathryn},
  author={Meyerhoff, Robert},
  author={Wu, Chenxi},
  journal={Advances in Mathematics},
  volume={482},
  pages={110636},
  year={2025},
  publisher={Elsevier}
}

	

\bib{GP}{article}{ ,
title={Conway Rational Tangles and the Thompson Group},
author={Grymski, Ariana},
author={Peters, Emily},
journal = {Journal of Knot Theory and Its Ramifications},
volume = {34},
number = {10},
pages = {2450044},
year = {2025},
doi = {10.1142/S0218216524500445}
}




\bib{Nesh}{article}{
  title={Subproduct systems with quantum group symmetry},
  author={Habbestad, Erik},
  author={Neshveyev, Sergey},
  journal={Journal of Noncommutative Geometry},
  volume={18},
  number={1},
  pages={93--121},
  year={2023}
}
\bib{Nesh2}{article}{
  title={Subproduct systems with quantum group symmetry II},
  author={Habbestad, Erik},
  author={Neshveyev, Sergey},
  journal={Trans. Amer. Math. Soc.}, 
    volume={378},
   pages={5159--5185 },
  year={2025}
}



\bib{Ly}{article}{
  title={Presentation of the Motzkin monoid},
  author={Hatch, Kris},
  author={Ly, M.},
    author={Posner, Eliezer},
  journal={preprint arXiv:1301.4518},
  year={2013}
}




\bib{HIG}{book}{%higman1974finitely,
title={Finitely presented infinite simple groups},
author={Higman, Graham},
volume={8},
year={1974},
publisher={Department of Pure Mathematics, Department of Mathematics, IAS, Australian}
}

\bib{Hornik}{article}{
  title={Approximation capabilities of multilayer feedforward networks},
  author={Hornik, Kurt},
  journal={Neural networks},
  volume={4},
  number={2},
  pages={251--257},
  year={1991},
  publisher={Elsevier}
}



\bib{Jonespolynomial}{article}{ 
  title={A polynomial invariant for links from Von Neumann algebras},
AUTHOR = {Jones, Vaughan F. R.},
  journal={Bulletin of the American Mathematical Society},
  volume={12},
  year={1985}
}
		
\bib{jo2}{article}{
AUTHOR = {Jones, Vaughan F. R.},
title={Planar Algebras I},
journal={New Zealand Journal of Mathematics},
volume={52},
pages={1-107},
note={preprint \href{http://arxiv.org/abs/9909027}{arXiv:9909027}},
year={2021},
}

		

\bib{Jo14}{article}{
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {Some unitary representations of {T}hompson's groups {$F$} and {$T$}},
JOURNAL = {J. Comb. Algebra},
FJOURNAL = {Journal of Combinatorial Algebra},
VOLUME = {1},
YEAR = {2017},
NUMBER = {1},
PAGES = {1--44},
ISSN = {2415-6302},
MRCLASS = {57M25 (20F38 46L37 81T40)},
MRNUMBER = {3589908},
MRREVIEWER = {Conchita Mart\'{\i}nez-P\'{e}rez},
DOI = {10.4171/JCA/1-1-1},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/JCA/1-1-1},
}





\bib{Jo16}{article}{
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {A no-go theorem for the continuum limit of a periodic quantum
  spin chain},
JOURNAL = {Comm. Math. Phys.},
FJOURNAL = {Communications in Mathematical Physics},
VOLUME = {357},
YEAR = {2018},
NUMBER = {1},
PAGES = {295--317},
ISSN = {0010-3616},
MRCLASS = {82B10 (81R12)},
MRNUMBER = {3764571},
MRREVIEWER = {Lawrence E. Thomas},
DOI = {10.1007/s00220-017-2945-3},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s00220-017-2945-3},
}

		




\bib{Jo18}{article}{
AUTHOR = {Jones, Vaughan F. R.},
TITLE = {On the construction of knots and links from Thompson's       groups},
BOOKTITLE = {Knots, low-dimensional topology and applications},
SERIES = {Springer Proc. Math. Stat.},
VOLUME = {284},
PAGES = {43--66},
PUBLISHER = {Springer, Cham},
YEAR = {2019},
MRCLASS = {57M25 (20F36 20F38 22D10 57M27)},
MRNUMBER = {3986040},
DOI = {10.1007/978-3-030-16031-9\_3},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/978-3-030-16031-9_3},
}
		




		
\bib{Jo19}{incollection}{
AUTHOR = {Jones, Vaughan F. R.},
title={Irreducibility of the Wysiwyg representations of Thompson's groups},
booktitle={Representation Theory, Mathematical Physics, and Integrable Systems},
pages={411--430},
year={2021},
publisher={Springer}
}

\bib{Jo21}{article}{
  title={Motzkin algebras and the $A_n$ tensor categories of bimodules},
  author={Jones, Vaughan F. R.},
  author={Yang, Jun},
  journal={International Journal of Mathematics},
  volume={32},
  number={10},
  pages={2150077},
  year={2021},
  publisher={World Scientific}
}

\bib{KS}{article}{
  title={Operator algebras of monomial ideals in noncommuting variables},
  author={Kakariadis, Evgenios TA},
  author={Shalit, Orr Moshe},
  journal={Journal of Mathematical Analysis and Applications},
  volume={472},
  number={1},
  pages={738--813},
  year={2019},
  publisher={Elsevier}
}


\bib{Kodama}{article}{
title={The $p$-colorable subgroup of Thompson's group},
author={Kodama, Yuya and Takano, Akihiro},
journal={preprint arXiv:2302.10060},
year={2023}
}


\bib{KKW}{article}{,
  title={Markovianity and the Thompson monoid $F^+$},
author={K{\"o}stler, Claus}, 
author={Krishnan, Arundhathi},
  author={Wills, Stephen J.},
  journal={Journal of Functional Analysis},
  volume={284},
  number={6},
  pages={109818},
  year={2023},
  publisher={Elsevier}
}


\bib{Kostler}{article}{,
title={Markovianity and the Thompson group F},
author={K{\"o}stler, Claus}, 
author={Krishnan, Arundhathi},
journal={SIGMA. Symmetry, Integrability and Geometry: Methods and Applications},
volume={18},
pages={083},
year={2022},
publisher={SIGMA. Symmetry, Integrability and Geometry: Methods and Applications}
}


\bib{Kri}{article}{
title={A central limit theorem in the framework of the Thompson group $F$},
author={Krishnan, Arundhathi},
journal={preprint arXiv:2309.05626},
year={2023}
}


\bib{LarsenLi}{article}{
  title={The 2-adic ring C$^*$-algebra of the integers and its representations},
  author={Larsen, Nadia S},
  author={Li, Xin},
  journal={Journal of Functional Analysis},
  volume={262},
  number={4},
  pages={1392--1426},
  year={2012},
  publisher={Elsevier}
}

\bib{LLPS}{article}{
  title={Multilayer feedforward networks with a nonpolynomial activation function can approximate any function},
  author={Leshno, Moshe},
  author={Lin, Vladimir Ya},
  author={Pinkus, Allan},
  author={Schocken, Shimon},
  journal={Neural networks},
  volume={6},
  number={6},
  pages={861--867},
  year={1993},
  publisher={Elsevier}
}




\bib{Ma}{article}{
AUTHOR = {Mackey, George W.},
TITLE = {The theory of unitary group representations},
NOTE = {Based on notes by James M. G. Fell and David B. Lowdenslager of lectures given at the University of Chicago, Chicago, Ill., 1955, Chicago Lectures in Mathematics},
PUBLISHER = {University of Chicago Press, Chicago, Ill.-London},
YEAR = {1976},
PAGES = {x+372},
MRCLASS = {22-02},
MRNUMBER = {0396826},
}



\bib{MPS}{article}{
AUTHOR = {Morrison, Scott},
AUTHOR = {Peters, Emily},
AUTHOR = {Snyder, Noah},
TITLE = {Categories generated by a trivalent vertex},
JOURNAL = {Selecta Math. (N.S.)},
FJOURNAL = {Selecta Mathematica. New Series},
VOLUME = {23},
YEAR = {2017},
NUMBER = {2},
PAGES = {817--868},
ISSN = {1022-1824},
MRCLASS = {18D10 (05C10 57M27)},
MRNUMBER = {3624901},
MRREVIEWER = {Marko \v{Z}ivkovi\'{c}},
DOI = {10.1007/s00029-016-0240-3},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s00029-016-0240-3},
}

\bib{NR}{article}{
AUTHOR = {Nikkel, Jordan},
AUTHOR = {Ren, Yunxiang},
TITLE = {On {J}ones' subgroup of {R}. {T}hompson's group {$T$}},
JOURNAL = {Internat. J. Algebra Comput.},
FJOURNAL = {International Journal of Algebra and Computation},
VOLUME = {28},
YEAR = {2018},
NUMBER = {5},
PAGES = {877--903},
ISSN = {0218-1967},
MRCLASS = {20F65 (20F05)},
MRNUMBER = {3844705},
MRREVIEWER = {J\"{o}rg Lehnert},
DOI = {10.1142/S0218196718500388},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1142/S0218196718500388},
}
		
		
\bib{Pacini24}{inproceedings}{ 
  title={A characterization theorem for equivariant networks with point-wise activations},
  author={Pacini, Marco},
  author={Dong, Xiaowen},
  author={Lepri, Bruno},
  author={Santin, Gabriele},
  booktitle={International Conference on Learning Representations},
  volume={2024},
  pages={38196--38216},
  year={2024}
}
		
\bib{Popescu}{article}{
  title={Operator theory on noncommutative varieties},
  author={Popescu, Gelu},
  journal={Indiana University mathematics journal},
  pages={389--442},
  year={2006},
  publisher={JSTOR}
}

\bib{Popescu2}{article}{
  title={Operator theory on noncommutative varieties, II},
  author={Popescu, Gelu},
  journal={Proceedings of the American Mathematical Society},
  volume={135},
  number={7},
  pages={2151--2164},
  year={2007}
}
		
		
\bib{RS}{article}{
title={Regular Isotopy Classes of Link Diagrams From Thompson's Groups},
author={Raghavan, Rushil},
author={Sweeney, Dennis},
journal={preprint arXiv arXiv:2008.11052},
year={2020}
}

\bib{Ren}{article}{
AUTHOR = {Ren, Yunxiang},
TITLE = {From skein theory to presentations for {T}hompson group},
JOURNAL = {J. Algebra},
FJOURNAL = {Journal of Algebra},
VOLUME = {498},
YEAR = {2018},
PAGES = {178--196},
ISSN = {0021-8693},
MRCLASS = {43A10 (20F65)},
MRNUMBER = {3754410},
MRREVIEWER = {M\u{a}d\u{a}lina Roxana Buneci},
DOI = {10.1016/j.jalgebra.2017.11.018},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jalgebra.2017.11.018},
}

\bib{RockafellarConvex}{book}{
  author    = {R. Tyrrell Rockafellar},
  title     = {Convex Analysis},
  series    = {Princeton Mathematical Series},
  volume    = {28},
  publisher = {Princeton University Press},
  year      = {1970}
}

\bib{Sav}{article}{
AUTHOR = {Savchuk, Dmytro},
TITLE = {Some graphs related to Thompson's group {$F$}},
BOOKTITLE = {Combinatorial and geometric group theory},
SERIES = {Trends Math.},
PAGES = {279--296},
PUBLISHER = {Birkh\"{a}user/Springer Basel AG, Basel},
YEAR = {2010},
MRCLASS = {20F65},
MRNUMBER = {2744025},
MRREVIEWER = {Fran\c{c}ois Dahmani},
DOI = {10.1007/978-3-7643-9911-5\_12},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/978-3-7643-9911-5_12},
}
			
			
	
\bib{Sav2}{article}{
AUTHOR = {Savchuk, Dmytro},
TITLE = {Schreier graphs of actions of Thompson's group {$F$} on the
unit interval and on the Cantor set},
JOURNAL = {Geom. Dedicata},
FJOURNAL = {Geometriae Dedicata},
VOLUME = {175},
YEAR = {2015},
PAGES = {355--372},
ISSN = {0046-5755},
MRCLASS = {20F65 (37C85)},
MRNUMBER = {3323646},
MRREVIEWER = {Ariadna Fossas},
DOI = {10.1007/s10711-014-9951-9},
URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s10711-014-9951-9},
}

\bib{Shalit}{article}{
  title={Subproduct systems},
  author={Shalit, Orr},
  author={Solel, Baruch},
  journal={Documenta Mathematica},
  volume={14},
  pages={801--868},
  year={2009}
}
	
	
	
\bib{Skeide}{article}{
title={Algebraic central limit theorems: A personal view on one of Wilhelm’s legacies},
author={Skeide, Michael},
journal={Infinite Dimensional Analysis, Quantum Probability and Related Topics},
volume={25},
number={04},
pages={2240003},
year={2022},
publisher={World Scientific}
}


\bib{Stallings}{article}{ 
title={Topology of finite graphs},
author={Stallings, John R.},
journal={Invent. Math.},
volume={71},
number={3},
pages={551--65},
year={1983}
}

\bib{Thomas18}{article}{ 
  title={Tensor field networks: Rotation-and translation-equivariant neural networks for 3d point clouds},
  author={Thomas, Nathaniel},
  author={Smidt, Tess},
  author={Kearnes, Steven},
  author={Yang, Lusann},
  author={Li, Li},
  author={Kohlhoff, Kai},
  author={Riley, Patrick},
  journal={preprint arXiv:1802.08219},
  year={2018}
}


\bib{Viselter12}{article}{ 
  title={Cuntz-Pimsner algebras for subproduct systems},
  author={Viselter, Ami},
  journal={International Journal of Mathematics},
  volume={23},
  number={08},
  pages={1250081},
  year={2012},
  publisher={World Scientific}
}
	
	
\bib{Voi}{book}{
title={Free random variables},
author={Voiculescu, Dan V.},
author={Dykema, Ken J.},
author={Nica, Alexandru},
number={1},
year={1992},
publisher={American Mathematical Soc.}
}

\bib{deepsets}{article}{ 
  title={Deep sets},
  author={Zaheer, Manzil},
  author={Kottur, Satwik},
  author={Ravanbakhsh, Siamak},
  author={Poczos, Barnabas},
  author={Salakhutdinov, Russ R},
  author={Smola, Alexander J},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}



\end{biblist}
%\end{bibdiv}
